Multi-Grid Graph Neural Networks with Self-Attention for Computational Mechanics

Advancement in finite element methods have become essential in various disciplines, and in particular for Computational Fluid Dynamics (CFD), driving research efforts for improved precision and efficiency. While Convolutional Neural Networks (CNNs) have found success in CFD by mapping meshes into images, recent attention has turned to leveraging Graph Neural Networks (GNNs) for direct mesh processing. This paper introduces a novel model merging Self-Attention with Message Passing in GNNs, achieving a 15\% reduction in RMSE on the well known flow past a cylinder benchmark. Furthermore, a dynamic mesh pruning technique based on Self-Attention is proposed, that leads to a robust GNN-based multigrid approach, also reducing RMSE by 15\%. Additionally, a new self-supervised training method based on BERT is presented, resulting in a 25\% RMSE reduction. The paper includes an ablation study and outperforms state-of-the-art models on several challenging datasets, promising advancements similar to those recently achieved in natural language and image processing. Finally, the paper introduces a dataset with meshes larger than existing ones by at least an order of magnitude. Code and Datasets will be released at https://github.com/DonsetPG/multigrid-gnn.

==> background.tex <==
The success of Convolutional Neural Networks (CNN) in image processing \cite{imagenet, alexnet} prompted their direct application to Computational Fluid Dynamics (CFD). One significant application involves mapping meshes or velocity and pressure fields into images to exploit such CNNs. \cite{Tompson2016} conducted 3D-fluid simulations employing a CNN that forecasts subsequent images based on preceding ones. Similarly, both \cite{Thuerey2018} and \cite{Chen2019} utilized a U-net architecture to predict pressure and velocity fields given solely a shape as input. However, these approaches were not applied to sequences of meshes/images and cannot leverage the power of unstructured grids.

Concurrently, \cite{Battaglia2016} and \cite{sanchezgonzalez2020learning} constructed a framework based on Graph Neural Networks (GNNs) that made it possible to process unstructured grids or meshes directly. \cite{pfaff2021learning} achieved state-of-the-art results with such an approach, albeit restricted to small meshes (under 4000 nodes). To overcome this limitation, \cite{Yang2022amgnet, taghibakhshi2023mggnn,lino2021simulating} employ multiple graph coarsening stages, while \cite{Fortunato2022} builds and operates with two graphs of different refinement stages from the start. Returning to CNNs, this MultiGrid approach can be put in parallel with U-net architectures \cite{ronneberger2015unet,lin2017feature}. In its simplest form, devoid of skip-connections, a U-net can be likened to a basic multigrid V-cycle for images. With the incorporation of skip-connections, a more intricate W-cycle emerges.

Beginning with Natural Language Processing (NLP), Transformers \cite{vaswani2023attention} achieved state-of-the-art results by replacing CNN and Recurrent layers with Self-Attention and Multi-Layer Perceptron (MLP). They now achieve state-of-the-art results in Computer Vision and Image Generation \cite{dosovitskiy2021image, arnab2021vivit} as well. While Transformers were introduced for GNNs before\cite{yun2020graph,müller2023attending,veličković2018graph}, those operations were primarily created for spatial fashion and not for sequences of graphs. \cite{shi2021masked} introduce a Self-Attention mechanism to coarsen a graph, bridging the gap with the MultiGrid approaches seen above.

\cite{devlin2019bert} constructed a framework where tokens from a sentence are being masked before being passed to a model. This method is now a key element of any LLM training. \cite{he2021masked} adapts the same approach for images, while masking a much larger amounts of information (up to 85\% of an image). \cite{Hu2019} masked a fraction of the nodes' features, but keep the structural integrity of the graphs they work with. \cite{Tan2022} masked some subset of edges before reconstructing the final graph with an Auto Encoder architecture, similar to \cite{he2021masked}.

In this paper, we develop a dynamic MultiGrid approach to spatially process meshes. Our architecture can autoregressively predict full CFD simulations from a minimal amount of inputs. We also present a novel pre-training task for Graph that leads in a boost of performance.
